Weak-Lensing Mass Calibration of the Atacama Cosmology Telescope Equatorial Sunyaev-Zeldovich Cluster Sample with the Canada-France-Hawaii Telescope Stripe 82 Survey

Mass calibration uncertainty is the largest systematic effect for using clusters of galaxies to constrain cosmological parameters. We present weak lensing mass measurements from the Canada-France-Hawaii Telescope Stripe 82 Survey for galaxy clusters selected through their high signal-to-noise thermal Sunyaev-Zeldovich (tSZ) signal measured with the Atacama Cosmology Telescope (ACT). For a sample of 9 ACT clusters with a tSZ signal-to-noise greater than five the average weak lensing mass is $\left(4.8\pm0.8\right)\,\times10^{14}\,\mathrm{M}_\odot$, consistent with the tSZ mass estimate of $\left(4.70\pm1.0\right)\,\times10^{14}\,\mathrm{M}_\odot$ which assumes a universal pressure profile for the cluster gas. Our results are consistent with previous weak-lensing measurements of tSZ-detected clusters from the Planck satellite. When comparing our results, we estimate the Eddington bias correction for the sample intersection of Planck and weak-lensing clusters which was previously excluded.

==> makefile <==
# Makefile to produce the article.
LATEX  =  TEXINPUTS=.//: BSTINPUTS=.//: latex
PDFLATEX  = pdflatex -shell-escape 
DVIPS  =  dvips
PSPDF  =  ps2pdf
FIGURES = figures/

.PRECIOUS: $(FIGURES)

default: cs82_act.pdf

%.pdf : $(FIGURES) %.tex
	$(PDFLATEX) $*.tex	
	TEXINPUTS=:.// BSTINPUTS=:.// bibtex $*
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
	$(PDFLATEX) $*.tex
#	$(DVIPS) -o $*.ps $*.dvi
#	$(PSPDF) $*.ps $*.pdf
	make clean

clean:
	rm -f *.log *.toc *.aux *.bak *.blg *.obj *.out

realclean:
	rm -f *.log *.toc *.aux *.obj *.bak *.bbl *.blg *.brf \
              *~ */*~ *.bak */*.bak 

